Revisiting the Primacy of English in Zero-shot Cross-lingual Transfer

Despite their success, large pre-trained multilingual models have not completely alleviated the need for labeled data, which is cumbersome to collect for all target languages. Zero-shot cross-lingual transfer is emerging as a practical solution: pre-trained models later fine-tuned on one transfer language exhibit surprising performance when tested on many target languages. English is the dominant source language for transfer, as reinforced by popular zero-shot benchmarks. However, this default choice has not been systematically vetted. In our study, we compare English against other transfer languages for fine-tuning, on two pre-trained multilingual models (mBERT and mT5) and multiple classification and question answering tasks. We find that other high-resource languages such as German and Russian often transfer more effectively, especially when the set of target languages is diverse or unknown a priori. Unexpectedly, this can be true even when the training sets were automatically translated from English. This finding can have immediate impact on multilingual zero-shot systems, and should inform future benchmark designs.

==> tables/pawsx_mbert.tex <==
\begin{tabularx}{\linewidth}{|l|YYYY|YYY|YYY|}
\toprule
\multicolumn{1}{|c|}{Train} & \multicolumn{4}{c|}{Latin Scripts} & \multicolumn{3}{c|}{CJK} & \multicolumn{3}{c|}{Averages} \\
\multicolumn{1}{|c|}{Data} & \lang{en}{O} & \lang{de}{HT} & \lang{es}{HT} & \lang{fr}{HT} & \lang{zh}{HT} & \lang{ja}{HT} & \lang{ko}{HT} & \multicolumn{1}{c}{$\rightarrow$\footnotesize{Latin}} & \multicolumn{1}{c}{$\rightarrow$\footnotesize{CJK}} & \multicolumn{1}{c|}{$\rightarrow$\footnotesize{All}} \\
\midrule
\multicolumn{11}{l}{} \\[-3pt]
\multicolumn{11}{l}{\textbf{mBERT}} \\
\midrule
\lang{en}{O} & 100.0 & 97.8 & 97.4 & 98.3 & 93.6 & 94.8 & 93.2 & 98.4 & 93.9 & 96.4 \\
\midrule
\lang{de}{MT} & \cellcolor{cfbd7c5} \textcolor{c000000}{-1.7} & \cellcolor{cb9d9ea} \textcolor{c000000}{+2.2} & \cellcolor{ceef4f7} \textcolor{c000000}{+0.5} & \cellcolor{cf8f9f9} \textcolor{c000000}{+0.1} & \cellcolor{cbedceb} \textcolor{c000000}{+2.1} & \cellcolor{c9ac7df} \textcolor{c000000}{+2.9} & \cellcolor{ca5cde3} \textcolor{c000000}{+2.7} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.3} & \cellcolor{cabd2e5} \textcolor{c000000}{+2.6} & \cellcolor{cddecf4} \textcolor{c000000}{+1.3} \\
\lang{es}{MT} & \cellcolor{cfde9dd} \textcolor{c000000}{-1.0} & \cellcolor{cfaf7f6} \textcolor{c000000}{-0.1} & \cellcolor{ca7cfe4} \textcolor{c000000}{+2.6} & \cellcolor{cd8e9f3} \textcolor{c000000}{+1.4} & \cellcolor{ce6f0f6} \textcolor{c000000}{+0.9} & \cellcolor{ce0edf5} \textcolor{c000000}{+1.2} & \cellcolor{ce0edf5} \textcolor{c000000}{+1.1} & \cellcolor{ce9f2f6} \textcolor{c000000}{+0.7} & \cellcolor{ce2eef5} \textcolor{c000000}{+1.1} & \cellcolor{ce6f0f6} \textcolor{c000000}{+0.9} \\
\lang{fr}{MT} & \cellcolor{cfbd5c3} \textcolor{c000000}{-1.7} & \cellcolor{cfbf0e9} \textcolor{c000000}{-0.6} & \cellcolor{ccce3ef} \textcolor{c000000}{+1.7} & \cellcolor{ccee4f0} \textcolor{c000000}{+1.7} & \cellcolor{cc0ddec} \textcolor{c000000}{+2.0} & \cellcolor{cb7d9e9} \textcolor{c000000}{+2.3} & \cellcolor{cdaeaf3} \textcolor{c000000}{+1.3} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.3} & \cellcolor{cc5e0ed} \textcolor{c000000}{+1.9} & \cellcolor{ce4eff5} \textcolor{c000000}{+1.0} \\
\midrule
\lang{zh}{MT} & \cellcolor{cba5868} \textcolor{c000000}{-5.1} & \cellcolor{cf4b7a1} \textcolor{c000000}{-2.6} & \cellcolor{cf2b49e} \textcolor{c000000}{-2.7} & \cellcolor{ce59587} \textcolor{c000000}{-3.4} & \cellcolor{c506e90} \textcolor{c000000}{+6.4} & \cellcolor{c527195} \textcolor{c000000}{+5.9} & \cellcolor{c608dbc} \textcolor{c000000}{+5.0} & \cellcolor{ce59587} \textcolor{c000000}{-3.5} & \cellcolor{c54769b} \textcolor{c000000}{+5.8} & \cellcolor{ceef4f7} \textcolor{c000000}{+0.5} \\
\lang{ja}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-13.8} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-10.2} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-10.8} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-10.5} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.3} & \cellcolor{c5d87b3} \textcolor{c000000}{+5.2} & \cellcolor{ccce3ef} \textcolor{c000000}{+1.7} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-11.3} & \cellcolor{cb4d7e8} \textcolor{c000000}{+2.4} & \cellcolor{cab5466} \textcolor{cf1f1f1}{-5.4} \\
\lang{ko}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-8.4} & \cellcolor{cd47475} \textcolor{c000000}{-4.3} & \cellcolor{cb35667} \textcolor{c000000}{-5.3} & \cellcolor{ca55265} \textcolor{cf1f1f1}{-5.6} & \cellcolor{cbcdbeb} \textcolor{c000000}{+2.1} & \cellcolor{c567aa1} \textcolor{c000000}{+5.6} & \cellcolor{c506e90} \textcolor{c000000}{+6.8} & \cellcolor{c994e63} \textcolor{cf1f1f1}{-5.9} & \cellcolor{c6292c2} \textcolor{c000000}{+4.9} & \cellcolor{cfde3d4} \textcolor{c000000}{-1.3} \\
\bottomrule
\end{tabularx}

\vspace{5pt}

==> tables/pawsx_mt5.tex <==
\begin{tabularx}{\linewidth}{|l|YYYY|YYY|YYY|}
% \toprule
% \multicolumn{1}{|c|}{Train} & \multicolumn{4}{c|}{Latin Scripts} & \multicolumn{3}{c|}{CJK} & \multicolumn{3}{c|}{Averages} \\
% \multicolumn{1}{|c|}{Data} & \lang{en}{O} & \lang{de}{HT} & \lang{es}{HT} & \lang{fr}{HT} & \lang{zh}{HT} & \lang{ja}{HT} & \lang{ko}{HT} & \multicolumn{1}{c}{$\rightarrow$\footnotesize{Latin}} & \multicolumn{1}{c}{$\rightarrow$\footnotesize{CJK}} & \multicolumn{1}{c|}{$\rightarrow$\footnotesize{All}} \\
% \midrule
% \multicolumn{11}{|c|}{\makecell{{} \\[-5pt] Relative Zero-Shot Abilities (\autoref{eq:single-ability})}} \\
\multicolumn{11}{l}{\textbf{mT5}} \\
\midrule
\lang{en}{O} & 100.0 & 98.8 & 99.6 & 99.1 & 95.3 & 97.5 & 93.9 & 99.4 & 95.6 & 97.7 \\
\midrule
% \multicolumn{11}{|c|}{\makecell{{} \\[-5pt] Zero-Shot Advantages over \lang{en}{O} (\autoref{eq:advantage})}} \\
% \midrule
\lang{de}{MT} & \cellcolor{cfaf4f0} \textcolor{c000000}{-0.2} & \cellcolor{cbfdceb} \textcolor{c000000}{+1.2} & \cellcolor{cd8e9f2} \textcolor{c000000}{+0.8} & \cellcolor{ce1eef4} \textcolor{c000000}{+0.6} & \cellcolor{c63a2cb} \textcolor{c000000}{+2.6} & \cellcolor{cfaf4f0} \textcolor{c000000}{-0.2} & \cellcolor{c90c2dd} \textcolor{c000000}{+1.9} & \cellcolor{ce0edf4} \textcolor{c000000}{+0.6} & \cellcolor{cb3d6e8} \textcolor{c000000}{+1.4} & \cellcolor{ccee4f0} \textcolor{c000000}{+1.0} \\
\lang{es}{MT} & \cellcolor{cf3af95} \textcolor{c000000}{-1.7} & \cellcolor{cfbd1bd} \textcolor{c000000}{-1.1} & \cellcolor{ce9f1f6} \textcolor{c000000}{+0.4} & \cellcolor{cfaf4f0} \textcolor{c000000}{-0.2} & \cellcolor{cf7f8f8} \textcolor{c000000}{+0.0} & \cellcolor{cdd7e70} \textcolor{c000000}{-2.4} & \cellcolor{cf9f6f3} \textcolor{c000000}{-0.1} & \cellcolor{cfce7da} \textcolor{c000000}{-0.6} & \cellcolor{cfde1d0} \textcolor{c000000}{-0.8} & \cellcolor{cfde4d5} \textcolor{c000000}{-0.7} \\
\lang{fr}{MT} & \cellcolor{cfaceb8} \textcolor{c000000}{-1.2} & \cellcolor{cfce7db} \textcolor{c000000}{-0.6} & \cellcolor{cd2e6f1} \textcolor{c000000}{+0.9} & \cellcolor{cd4e7f1} \textcolor{c000000}{+0.9} & \cellcolor{ce6f0f5} \textcolor{c000000}{+0.5} & \cellcolor{cf8c0a7} \textcolor{c000000}{-1.4} & \cellcolor{c93c3dd} \textcolor{c000000}{+1.8} & \cellcolor{cf8f8f8} \textcolor{c000000}{+0.0} & \cellcolor{cedf3f7} \textcolor{c000000}{+0.3} & \cellcolor{cf3f6f8} \textcolor{c000000}{+0.1} \\
\midrule
\lang{zh}{MT} & \cellcolor{cf7bfa5} \textcolor{c000000}{-1.5} & \cellcolor{cf9f6f5} \textcolor{c000000}{-0.1} & \cellcolor{ce0edf4} \textcolor{c000000}{+0.6} & \cellcolor{cf2f5f7} \textcolor{c000000}{+0.2} & \cellcolor{c375981} \textcolor{cf1f1f1}{+4.7} & \cellcolor{c426f9f} \textcolor{c000000}{+3.6} & \cellcolor{c375981} \textcolor{cf1f1f1}{+4.9} & \cellcolor{cfaf4f0} \textcolor{c000000}{-0.2} & \cellcolor{c375981} \textcolor{cf1f1f1}{+4.4} & \cellcolor{c98c6df} \textcolor{c000000}{+1.8} \\
\lang{ja}{MT} & \cellcolor{cf4b297} \textcolor{c000000}{-1.7} & \cellcolor{cfce9de} \textcolor{c000000}{-0.5} & \cellcolor{cf9f6f5} \textcolor{c000000}{-0.1} & \cellcolor{cf9f6f5} \textcolor{c000000}{-0.1} & \cellcolor{c375981} \textcolor{cf1f1f1}{+4.5} & \cellcolor{c63a2cb} \textcolor{c000000}{+2.5} & \cellcolor{c375981} \textcolor{cf1f1f1}{+5.5} & \cellcolor{cfce7db} \textcolor{c000000}{-0.6} & \cellcolor{c375981} \textcolor{cf1f1f1}{+4.2} & \cellcolor{cb1d5e7} \textcolor{c000000}{+1.5} \\
\lang{ko}{MT} & \cellcolor{cfad0ba} \textcolor{c000000}{-1.1} & \cellcolor{cfaf0ea} \textcolor{c000000}{-0.3} & \cellcolor{cebf2f6} \textcolor{c000000}{+0.4} & \cellcolor{cf1f5f7} \textcolor{c000000}{+0.2} & \cellcolor{c497db2} \textcolor{c000000}{+3.3} & \cellcolor{c3e6793} \textcolor{cf1f1f1}{+3.7} & \cellcolor{c375981} \textcolor{cf1f1f1}{+6.1} & \cellcolor{cfaf3ef} \textcolor{c000000}{-0.2} & \cellcolor{c375981} \textcolor{cf1f1f1}{+4.4} & \cellcolor{c9ac8e0} \textcolor{c000000}{+1.8} \\
\bottomrule
\end{tabularx}

==> tables/xnli_mbert.tex <==
\begin{tabularx}{\linewidth}{|c|YYYY|YYY|YYYYYYYY|YYYY|}
\toprule
\multicolumn{1}{|c|}{Train} & \multicolumn{4}{c|}{Latin/High = LH} & \multicolumn{3}{c|}{Latin/Low = LL} & \multicolumn{8}{c|}{Misc = M} & \multicolumn{4}{c|}{Averages} \\
\multicolumn{1}{|c|}{Data} & \langcol{en}{O} & \langcol{de}{HT} & \langcol{es}{HT} & \langcol{fr}{HT} & \langcol{sw}{HT} & \langcol{tr}{HT} & \langcol{vi}{HT} & \langcol{ar}{HT} & \langcol{bg}{HT} & \langcol{el}{HT} & \langcol{hi}{HT} & \langcol{ru}{HT} & \langcol{ur}{HT} & \langcol{th}{HT} & \langcol{zh}{HT} & $\rightarrow$\scriptsize{LH} & $\rightarrow$\scriptsize{LL} & $\rightarrow$\scriptsize{M} & $\rightarrow$\scriptsize{All} \\
\midrule
\multicolumn{20}{l}{} \\[-3pt]
\multicolumn{20}{l}{\footnotesize{\textbf{mBERT}}} \\
\midrule
\lang{en}{O} & 100.0 & 92.2 & 95.7 & 93.4 & 81.2 & 89.0 & 92.1 & 94.8 & 90.5 & 91.4 & 89.1 & 93.8 & 94.7 & 80.5 & 90.5 & 95.3 & 87.4 & 90.7 & 91.3 \\
\midrule
%\multicolumn{20}{|c|}{Zero-Shot Advantages over \lang{en}{O} (\autoref{eq:advantage})} \\
%\midrule
\lang{de}{MT} & \cellcolor{cf4b9a2} \textcolor{c000000}{-4.2} & \cellcolor{c6697c6} \textcolor{c000000}{+7.8} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.4} & \cellcolor{cddecf4} \textcolor{c000000}{+2.1} & \cellcolor{cf2b49e} \textcolor{c000000}{-4.5} & \cellcolor{cd8e9f3} \textcolor{c000000}{+2.3} & \cellcolor{ceff5f8} \textcolor{c000000}{+0.7} & \cellcolor{cd4e8f2} \textcolor{c000000}{+2.5} & \cellcolor{cd3e7f1} \textcolor{c000000}{+2.5} & \cellcolor{cdfedf4} \textcolor{c000000}{+2.0} & \cellcolor{ca7cfe4} \textcolor{c000000}{+4.4} & \cellcolor{ce5f0f6} \textcolor{c000000}{+1.5} & \cellcolor{cb2d6e8} \textcolor{c000000}{+4.0} & \cellcolor{c80b6d6} \textcolor{c000000}{+5.8} & \cellcolor{cc8e1ee} \textcolor{c000000}{+3.0} & \cellcolor{ce5f0f6} \textcolor{c000000}{+1.5} & \cellcolor{cfaf5f2} \textcolor{c000000}{-0.5} & \cellcolor{cc3dfed} \textcolor{c000000}{+3.2} & \cellcolor{cdfedf4} \textcolor{c000000}{+2.0} \\
\lang{es}{MT} & \cellcolor{cf8c7b0} \textcolor{c000000}{-3.6} & \cellcolor{ccee4f0} \textcolor{c000000}{+2.8} & \cellcolor{ca9d0e5} \textcolor{c000000}{+4.3} & \cellcolor{cd8e9f3} \textcolor{c000000}{+2.3} & \cellcolor{cfde9dd} \textcolor{c000000}{-1.7} & \cellcolor{cfbf0e9} \textcolor{c000000}{-1.0} & \cellcolor{cd4e8f2} \textcolor{c000000}{+2.5} & \cellcolor{ce0edf5} \textcolor{c000000}{+1.9} & \cellcolor{ce0edf5} \textcolor{c000000}{+1.9} & \cellcolor{cf9f9f9} \textcolor{c000000}{+0.1} & \cellcolor{cb7d9e9} \textcolor{c000000}{+3.8} & \cellcolor{cd1e6f1} \textcolor{c000000}{+2.6} & \cellcolor{cc0ddec} \textcolor{c000000}{+3.4} & \cellcolor{ca5cde3} \textcolor{c000000}{+4.5} & \cellcolor{cc3dfed} \textcolor{c000000}{+3.2} & \cellcolor{ce6f0f6} \textcolor{c000000}{+1.4} & \cellcolor{cf9f9f9} \textcolor{c000000}{-0.1} & \cellcolor{ccfe5f0} \textcolor{c000000}{+2.7} & \cellcolor{ce1eef5} \textcolor{c000000}{+1.8} \\
\lang{fr}{MT} & \cellcolor{cfbd4c1} \textcolor{c000000}{-3.0} & \cellcolor{ccae2ef} \textcolor{c000000}{+2.9} & \cellcolor{ce7f1f6} \textcolor{c000000}{+1.4} & \cellcolor{c75abd1} \textcolor{c000000}{+6.6} & \cellcolor{cfde7d9} \textcolor{c000000}{-1.9} & \cellcolor{cfde7da} \textcolor{c000000}{-1.8} & \cellcolor{cebf3f7} \textcolor{c000000}{+1.1} & \cellcolor{cc8e1ee} \textcolor{c000000}{+3.0} & \cellcolor{ce5f0f6} \textcolor{c000000}{+1.5} & \cellcolor{cfcede5} \textcolor{c000000}{-1.2} & \cellcolor{ce9f2f6} \textcolor{c000000}{+1.2} & \cellcolor{cdaeaf3} \textcolor{c000000}{+2.2} & \cellcolor{cb9d9ea} \textcolor{c000000}{+3.7} & \cellcolor{ccfe5f0} \textcolor{c000000}{+2.7} & \cellcolor{cbedceb} \textcolor{c000000}{+3.5} & \cellcolor{cdfedf4} \textcolor{c000000}{+2.0} & \cellcolor{cfbf1ea} \textcolor{c000000}{-0.9} & \cellcolor{cddecf4} \textcolor{c000000}{+2.1} & \cellcolor{ce6f0f6} \textcolor{c000000}{+1.5} \\
\midrule
\lang{sw}{MT} & \cellcolor{c9d4f64} \textcolor{cf1f1f1}{-9.7} & \cellcolor{cf7c1a8} \textcolor{c000000}{-3.9} & \cellcolor{cca5e6b} \textcolor{c000000}{-8.0} & \cellcolor{ceba592} \textcolor{c000000}{-5.1} & \cellcolor{c506e90} \textcolor{c000000}{+18.8} & \cellcolor{ce69788} \textcolor{c000000}{-5.7} & \cellcolor{cf4b9a2} \textcolor{c000000}{-4.3} & \cellcolor{cf5bba4} \textcolor{c000000}{-4.2} & \cellcolor{cefae9a} \textcolor{c000000}{-4.7} & \cellcolor{cfbd8c7} \textcolor{c000000}{-2.7} & \cellcolor{cfceee6} \textcolor{c000000}{-1.1} & \cellcolor{ceda895} \textcolor{c000000}{-5.0} & \cellcolor{cfad1bd} \textcolor{c000000}{-3.0} & \cellcolor{cf9f9f9} \textcolor{c000000}{+0.1} & \cellcolor{ce79b8b} \textcolor{c000000}{-5.5} & \cellcolor{cd97e7a} \textcolor{c000000}{-6.7} & \cellcolor{ccae2ef} \textcolor{c000000}{+2.9} & \cellcolor{cfaceb9} \textcolor{c000000}{-3.3} & \cellcolor{cfbd4c1} \textcolor{c000000}{-2.9} \\
\lang{tr}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-14.2} & \cellcolor{cfbd4c1} \textcolor{c000000}{-2.9} & \cellcolor{cf0b09b} \textcolor{c000000}{-4.6} & \cellcolor{cfcdbcb} \textcolor{c000000}{-2.5} & \cellcolor{cfde9dd} \textcolor{c000000}{-1.7} & \cellcolor{c506e90} \textcolor{c000000}{+11.0} & \cellcolor{cfbd5c3} \textcolor{c000000}{-2.9} & \cellcolor{cfaf4f1} \textcolor{c000000}{-0.5} & \cellcolor{cfaf8f7} \textcolor{c000000}{-0.1} & \cellcolor{cfde8dc} \textcolor{c000000}{-1.7} & \cellcolor{ca0cbe2} \textcolor{c000000}{+4.6} & \cellcolor{cfaf7f5} \textcolor{c000000}{-0.3} & \cellcolor{cd1e6f1} \textcolor{c000000}{+2.6} & \cellcolor{cd4e8f2} \textcolor{c000000}{+2.5} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.4} & \cellcolor{ce18e81} \textcolor{c000000}{-6.1} & \cellcolor{cdbebf4} \textcolor{c000000}{+2.2} & \cellcolor{cedf4f7} \textcolor{c000000}{+0.9} & \cellcolor{cfbf3ee} \textcolor{c000000}{-0.7} \\
\lang{vi}{MT} & \cellcolor{cbe5a69} \textcolor{c000000}{-8.4} & \cellcolor{cfcefe8} \textcolor{c000000}{-1.0} & \cellcolor{cfee6d8} \textcolor{c000000}{-2.0} & \cellcolor{cf2f6f8} \textcolor{c000000}{+0.6} & \cellcolor{cfbf1ea} \textcolor{c000000}{-0.9} & \cellcolor{cfbd8c7} \textcolor{c000000}{-2.7} & \cellcolor{c6495c5} \textcolor{c000000}{+7.9} & \cellcolor{cf2f6f8} \textcolor{c000000}{+0.6} & \cellcolor{ceff5f8} \textcolor{c000000}{+0.7} & \cellcolor{cf9f9f9} \textcolor{c000000}{-0.1} & \cellcolor{cc0ddec} \textcolor{c000000}{+3.4} & \cellcolor{cf9f9f9} \textcolor{c000000}{+0.0} & \cellcolor{ce5f0f6} \textcolor{c000000}{+1.6} & \cellcolor{c76acd1} \textcolor{c000000}{+6.5} & \cellcolor{ce6f0f6} \textcolor{c000000}{+1.5} & \cellcolor{cfbd8c7} \textcolor{c000000}{-2.7} & \cellcolor{ce6f0f6} \textcolor{c000000}{+1.4} & \cellcolor{ce2eef5} \textcolor{c000000}{+1.8} & \cellcolor{cf3f6f8} \textcolor{c000000}{+0.5} \\
\midrule
\lang{ar}{MT} & \cellcolor{ca55265} \textcolor{cf1f1f1}{-9.3} & \cellcolor{cfaf4f1} \textcolor{c000000}{-0.5} & \cellcolor{cfbd7c5} \textcolor{c000000}{-2.8} & \cellcolor{cf8f9f9} \textcolor{c000000}{+0.2} & \cellcolor{cfee6d8} \textcolor{c000000}{-2.0} & \cellcolor{cfde7da} \textcolor{c000000}{-1.8} & \cellcolor{cfbf3ee} \textcolor{c000000}{-0.7} & \cellcolor{c91c1dc} \textcolor{c000000}{+5.2} & \cellcolor{ce3eff5} \textcolor{c000000}{+1.6} & \cellcolor{cf5f7f9} \textcolor{c000000}{+0.3} & \cellcolor{ccfe5f0} \textcolor{c000000}{+2.7} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.4} & \cellcolor{cd1e6f1} \textcolor{c000000}{+2.6} & \cellcolor{ce5f0f6} \textcolor{c000000}{+1.5} & \cellcolor{cfaf7f6} \textcolor{c000000}{-0.2} & \cellcolor{cfad1bd} \textcolor{c000000}{-3.1} & \cellcolor{cfdeae0} \textcolor{c000000}{-1.5} & \cellcolor{ce2eef5} \textcolor{c000000}{+1.8} & \cellcolor{cfaf7f6} \textcolor{c000000}{-0.2} \\
\lang{bg}{MT} & \cellcolor{cce666f} \textcolor{c000000}{-7.6} & \cellcolor{ceef4f7} \textcolor{c000000}{+0.8} & \cellcolor{cfde4d6} \textcolor{c000000}{-2.1} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.5} & \cellcolor{cf9cbb6} \textcolor{c000000}{-3.4} & \cellcolor{cfcece2} \textcolor{c000000}{-1.4} & \cellcolor{cfaf8f7} \textcolor{c000000}{-0.1} & \cellcolor{ce6f0f6} \textcolor{c000000}{+1.5} & \cellcolor{c55789f} \textcolor{c000000}{+9.5} & \cellcolor{ceff5f8} \textcolor{c000000}{+0.7} & \cellcolor{cbcdbeb} \textcolor{c000000}{+3.5} & \cellcolor{ce5f0f6} \textcolor{c000000}{+1.5} & \cellcolor{ce1eef5} \textcolor{c000000}{+1.8} & \cellcolor{cdaeaf3} \textcolor{c000000}{+2.2} & \cellcolor{cdaeaf3} \textcolor{c000000}{+2.2} & \cellcolor{cfde3d4} \textcolor{c000000}{-2.1} & \cellcolor{cfdeade} \textcolor{c000000}{-1.6} & \cellcolor{ccce3ef} \textcolor{c000000}{+2.9} & \cellcolor{cf1f5f8} \textcolor{c000000}{+0.6} \\
\lang{el}{MT} & \cellcolor{ca35165} \textcolor{cf1f1f1}{-9.4} & \cellcolor{cfdeade} \textcolor{c000000}{-1.6} & \cellcolor{cf9cbb6} \textcolor{c000000}{-3.4} & \cellcolor{cfbf1ea} \textcolor{c000000}{-0.9} & \cellcolor{cfceee6} \textcolor{c000000}{-1.2} & \cellcolor{cfaf4f1} \textcolor{c000000}{-0.5} & \cellcolor{cfde7da} \textcolor{c000000}{-1.8} & \cellcolor{cfaf7f6} \textcolor{c000000}{-0.2} & \cellcolor{cf1f5f8} \textcolor{c000000}{+0.7} & \cellcolor{c5e89b5} \textcolor{c000000}{+8.6} & \cellcolor{cbedceb} \textcolor{c000000}{+3.5} & \cellcolor{cfbf4f0} \textcolor{c000000}{-0.6} & \cellcolor{cf5f7f9} \textcolor{c000000}{+0.4} & \cellcolor{c84b9d8} \textcolor{c000000}{+5.7} & \cellcolor{cfaf7f5} \textcolor{c000000}{-0.3} & \cellcolor{cf8c2aa} \textcolor{c000000}{-3.8} & \cellcolor{cfceee6} \textcolor{c000000}{-1.2} & \cellcolor{cdaeaf3} \textcolor{c000000}{+2.2} & \cellcolor{cf9f9f9} \textcolor{c000000}{-0.1} \\
\lang{hi}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-15.5} & \cellcolor{cf9cdb8} \textcolor{c000000}{-3.3} & \cellcolor{cbe5a69} \textcolor{c000000}{-8.4} & \cellcolor{cf9c8b2} \textcolor{c000000}{-3.6} & \cellcolor{cf5bba4} \textcolor{c000000}{-4.2} & \cellcolor{cfde4d6} \textcolor{c000000}{-2.1} & \cellcolor{cf9cab4} \textcolor{c000000}{-3.4} & \cellcolor{cfde4d6} \textcolor{c000000}{-2.0} & \cellcolor{cfde7d9} \textcolor{c000000}{-1.9} & \cellcolor{cf9c8b2} \textcolor{c000000}{-3.5} & \cellcolor{c506e90} \textcolor{c000000}{+10.9} & \cellcolor{cfcdece} \textcolor{c000000}{-2.4} & \cellcolor{c6a9cc9} \textcolor{c000000}{+7.5} & \cellcolor{cdfedf4} \textcolor{c000000}{+2.0} & \cellcolor{cfaf6f3} \textcolor{c000000}{-0.3} & \cellcolor{ccd646e} \textcolor{c000000}{-7.7} & \cellcolor{cfaceb9} \textcolor{c000000}{-3.2} & \cellcolor{ce8f1f6} \textcolor{c000000}{+1.3} & \cellcolor{cfee6d8} \textcolor{c000000}{-2.0} \\
\lang{ru}{MT} & \cellcolor{ce08c81} \textcolor{c000000}{-6.2} & \cellcolor{cddecf4} \textcolor{c000000}{+2.1} & \cellcolor{cfaf8f7} \textcolor{c000000}{-0.1} & \cellcolor{ce2eef5} \textcolor{c000000}{+1.8} & \cellcolor{cf4b7a1} \textcolor{c000000}{-4.3} & \cellcolor{cfbf4f0} \textcolor{c000000}{-0.6} & \cellcolor{cdfedf4} \textcolor{c000000}{+2.0} & \cellcolor{ce6f0f6} \textcolor{c000000}{+1.5} & \cellcolor{c9cc8e0} \textcolor{c000000}{+4.8} & \cellcolor{cddecf4} \textcolor{c000000}{+2.1} & \cellcolor{cb9d9ea} \textcolor{c000000}{+3.7} & \cellcolor{c7ab1d4} \textcolor{c000000}{+6.2} & \cellcolor{cabd2e5} \textcolor{c000000}{+4.3} & \cellcolor{ca5cde3} \textcolor{c000000}{+4.5} & \cellcolor{ccce3ef} \textcolor{c000000}{+2.9} & \cellcolor{cfbf4f0} \textcolor{c000000}{-0.6} & \cellcolor{cfbf0e9} \textcolor{c000000}{-1.0} & \cellcolor{cb9d9ea} \textcolor{c000000}{+3.7} & \cellcolor{ce4eff5} \textcolor{c000000}{+1.6} \\
\lang{ur}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-24.2} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-12.9} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-16.7} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-13.1} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-16.1} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-12.4} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-14.6} & \cellcolor{c994e63} \textcolor{cf1f1f1}{-9.8} & \cellcolor{c974d63} \textcolor{cf1f1f1}{-9.9} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-11.8} & \cellcolor{ce5f0f6} \textcolor{c000000}{+1.5} & \cellcolor{c994e63} \textcolor{cf1f1f1}{-9.8} & \cellcolor{c8dbedb} \textcolor{c000000}{+5.3} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-17.0} & \cellcolor{ca55265} \textcolor{cf1f1f1}{-9.4} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-16.7} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-14.3} & \cellcolor{cce666f} \textcolor{c000000}{-7.6} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-11.4} \\
\lang{th}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-24.1} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-11.3} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-13.8} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-11.3} & \cellcolor{cefac98} \textcolor{c000000}{-4.8} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-12.9} & \cellcolor{c994e63} \textcolor{cf1f1f1}{-9.8} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-10.6} & \cellcolor{ca55265} \textcolor{cf1f1f1}{-9.3} & \cellcolor{cb85868} \textcolor{c000000}{-8.6} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-10.0} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-11.4} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-12.6} & \cellcolor{c506e90} \textcolor{c000000}{+19.5} & \cellcolor{c9b4e63} \textcolor{cf1f1f1}{-9.7} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-15.1} & \cellcolor{ca95365} \textcolor{cf1f1f1}{-9.2} & \cellcolor{cda807b} \textcolor{c000000}{-6.6} & \cellcolor{ca35165} \textcolor{cf1f1f1}{-9.4} \\
\lang{zh}{MT} & \cellcolor{cd57676} \textcolor{c000000}{-7.0} & \cellcolor{cfbf1ea} \textcolor{c000000}{-0.9} & \cellcolor{cfcdac9} \textcolor{c000000}{-2.6} & \cellcolor{cf9f9f9} \textcolor{c000000}{+0.1} & \cellcolor{cad5466} \textcolor{c000000}{-9.0} & \cellcolor{cfaf8f7} \textcolor{c000000}{-0.1} & \cellcolor{ce3eff5} \textcolor{c000000}{+1.6} & \cellcolor{cf3f6f8} \textcolor{c000000}{+0.5} & \cellcolor{cf1f5f8} \textcolor{c000000}{+0.6} & \cellcolor{cfcece2} \textcolor{c000000}{-1.4} & \cellcolor{cc7e1ee} \textcolor{c000000}{+3.1} & \cellcolor{cf1f5f8} \textcolor{c000000}{+0.7} & \cellcolor{cbcdbeb} \textcolor{c000000}{+3.6} & \cellcolor{cfaf7f5} \textcolor{c000000}{-0.2} & \cellcolor{c55779d} \textcolor{c000000}{+9.5} & \cellcolor{cfcdac9} \textcolor{c000000}{-2.6} & \cellcolor{cfcddcc} \textcolor{c000000}{-2.5} & \cellcolor{cddecf4} \textcolor{c000000}{+2.0} & \cellcolor{cfaf8f7} \textcolor{c000000}{-0.1} \\
\midrule
\end{tabularx}

\vspace{5pt}

==> tables/xnli_mt5.tex <==
\begin{tabularx}{\linewidth}{|l|YYYY|YYY|YYYYYYYY|YYYY|}
% \toprule
% \multicolumn{1}{|l|}{Train} & \multicolumn{4}{c|}{Latin/High = LH} & \multicolumn{3}{c|}{Latin/Low = LL} & \multicolumn{8}{c|}{Misc = M} & \multicolumn{4}{c|}{Averages} \\
% \multicolumn{1}{|l|}{Data} & \lang{en}{O} & \lang{de}{HT} & \lang{es}{HT} & \lang{fr}{HT} & \lang{sw}{HT} & \lang{tr}{HT} & \lang{vi}{HT} & \lang{ar}{HT} & \lang{bg}{HT} & \lang{el}{HT} & \lang{hi}{HT} & \lang{ru}{HT} & \lang{ur}{HT} & \lang{th}{HT} & \lang{zh}{HT} & $\rightarrow$\scriptsize{LH} & $\rightarrow$\scriptsize{LL} & $\rightarrow$\scriptsize{M} & $\rightarrow$\scriptsize{All} \\
%\midrule
%\multicolumn{20}{|c|}{Relative Zero-Shot Abilities (\autoref{eq:single-ability})} \\
%\midrule
\multicolumn{20}{l}{\footnotesize{\textbf{mT5}}} \\
\midrule
\lang{en}{O} & 100.0 & 96.0 & 98.4 & 99.1 & 94.0 & 92.8 & 96.2 & 95.0 & 96.7 & 97.0 & 93.0 & 96.1 & 93.8 & 94.3 & 92.1 & 98.4 & 94.3 & 94.8 & 95.6 \\
\midrule
%\multicolumn{20}{|c|}{Zero-Shot Advantages over \lang{en}{O} (\autoref{eq:advantage})} \\
%\midrule
\lang{de}{MT} & \cellcolor{cfaceb9} \textcolor{c000000}{-1.6} & \cellcolor{c6495c5} \textcolor{c000000}{+4.0} & \cellcolor{ce8f1f6} \textcolor{c000000}{+0.6} & \cellcolor{cd1e6f1} \textcolor{c000000}{+1.3} & \cellcolor{c88bcd9} \textcolor{c000000}{+2.7} & \cellcolor{c91c1dc} \textcolor{c000000}{+2.6} & \cellcolor{cd4e8f2} \textcolor{c000000}{+1.2} & \cellcolor{c8fc0dc} \textcolor{c000000}{+2.7} & \cellcolor{cc7e1ee} \textcolor{c000000}{+1.5} & \cellcolor{cd3e7f1} \textcolor{c000000}{+1.3} & \cellcolor{c5980a9} \textcolor{c000000}{+4.5} & \cellcolor{c95c4de} \textcolor{c000000}{+2.5} & \cellcolor{c618fbe} \textcolor{c000000}{+4.1} & \cellcolor{c76acd1} \textcolor{c000000}{+3.2} & \cellcolor{c95c4de} \textcolor{c000000}{+2.5} & \cellcolor{cdbebf4} \textcolor{c000000}{+1.1} & \cellcolor{ca7cfe4} \textcolor{c000000}{+2.2} & \cellcolor{c86bad9} \textcolor{c000000}{+2.8} & \cellcolor{ca7cfe4} \textcolor{c000000}{+2.2} \\
\lang{es}{MT} & \cellcolor{cf7c1a8} \textcolor{c000000}{-2.0} & \cellcolor{cedf4f7} \textcolor{c000000}{+0.4} & \cellcolor{cc5e0ed} \textcolor{c000000}{+1.6} & \cellcolor{ce3eff5} \textcolor{c000000}{+0.8} & \cellcolor{cbcdbeb} \textcolor{c000000}{+1.8} & \cellcolor{cd1e6f1} \textcolor{c000000}{+1.3} & \cellcolor{ce3eff5} \textcolor{c000000}{+0.9} & \cellcolor{c9cc8e0} \textcolor{c000000}{+2.4} & \cellcolor{ce2eef5} \textcolor{c000000}{+0.9} & \cellcolor{ccfe5f0} \textcolor{c000000}{+1.3} & \cellcolor{c7bb3d5} \textcolor{c000000}{+3.0} & \cellcolor{cb9d9ea} \textcolor{c000000}{+1.8} & \cellcolor{ca0cbe2} \textcolor{c000000}{+2.3} & \cellcolor{c86bad9} \textcolor{c000000}{+2.8} & \cellcolor{cb5d8e9} \textcolor{c000000}{+1.9} & \cellcolor{cf4f7f8} \textcolor{c000000}{+0.2} & \cellcolor{cd1e6f1} \textcolor{c000000}{+1.3} & \cellcolor{cafd4e7} \textcolor{c000000}{+2.1} & \cellcolor{ccce3ef} \textcolor{c000000}{+1.4} \\
\lang{fr}{MT} & \cellcolor{ce79b8b} \textcolor{c000000}{-2.7} & \cellcolor{cfcece2} \textcolor{c000000}{-0.7} & \cellcolor{cfbf1ea} \textcolor{c000000}{-0.5} & \cellcolor{ce3eff5} \textcolor{c000000}{+0.9} & \cellcolor{cf2f6f8} \textcolor{c000000}{+0.3} & \cellcolor{cfbf2ed} \textcolor{c000000}{-0.4} & \cellcolor{cf7c1a8} \textcolor{c000000}{-2.0} & \cellcolor{cdbebf4} \textcolor{c000000}{+1.1} & \cellcolor{cfde7da} \textcolor{c000000}{-0.9} & \cellcolor{cfde7da} \textcolor{c000000}{-0.9} & \cellcolor{cedf4f7} \textcolor{c000000}{+0.5} & \cellcolor{cfaf7f5} \textcolor{c000000}{-0.1} & \cellcolor{cfbf1ea} \textcolor{c000000}{-0.4} & \cellcolor{cf6f8f9} \textcolor{c000000}{+0.1} & \cellcolor{cb5d8e9} \textcolor{c000000}{+1.9} & \cellcolor{cfdeae0} \textcolor{c000000}{-0.8} & \cellcolor{cfcece2} \textcolor{c000000}{-0.7} & \cellcolor{cf6f8f9} \textcolor{c000000}{+0.1} & \cellcolor{cfaf4f1} \textcolor{c000000}{-0.3} \\
\midrule
\lang{sw}{MT} & \cellcolor{cb65767} \textcolor{c000000}{-4.3} & \cellcolor{cfdeade} \textcolor{c000000}{-0.8} & \cellcolor{cf8c5ae} \textcolor{c000000}{-1.8} & \cellcolor{cfde3d4} \textcolor{c000000}{-1.1} & \cellcolor{c506e90} \textcolor{c000000}{+6.0} & \cellcolor{ccee4f0} \textcolor{c000000}{+1.4} & \cellcolor{cfcdac9} \textcolor{c000000}{-1.3} & \cellcolor{c82b8d7} \textcolor{c000000}{+2.9} & \cellcolor{cfde0d0} \textcolor{c000000}{-1.1} & \cellcolor{cfdeae0} \textcolor{c000000}{-0.8} & \cellcolor{c84b9d8} \textcolor{c000000}{+2.8} & \cellcolor{cfdeade} \textcolor{c000000}{-0.8} & \cellcolor{cd4e8f2} \textcolor{c000000}{+1.2} & \cellcolor{c8fc0dc} \textcolor{c000000}{+2.6} & \cellcolor{c80b6d6} \textcolor{c000000}{+2.9} & \cellcolor{cf7bfa7} \textcolor{c000000}{-2.0} & \cellcolor{cb2d6e8} \textcolor{c000000}{+2.0} & \cellcolor{cd4e8f2} \textcolor{c000000}{+1.2} & \cellcolor{cebf3f7} \textcolor{c000000}{+0.5} \\
\lang{tr}{MT} & \cellcolor{c9d4f64} \textcolor{cf1f1f1}{-4.8} & \cellcolor{cf6f8f9} \textcolor{c000000}{+0.1} & \cellcolor{cfad0bb} \textcolor{c000000}{-1.6} & \cellcolor{cfcece2} \textcolor{c000000}{-0.7} & \cellcolor{cd4e8f2} \textcolor{c000000}{+1.2} & \cellcolor{c506e90} \textcolor{c000000}{+7.2} & \cellcolor{cfbf2ed} \textcolor{c000000}{-0.4} & \cellcolor{ccce3ef} \textcolor{c000000}{+1.4} & \cellcolor{cf8f9f9} \textcolor{c000000}{+0.0} & \cellcolor{cf5f7f9} \textcolor{c000000}{+0.2} & \cellcolor{c55789f} \textcolor{c000000}{+4.7} & \cellcolor{ce5f0f6} \textcolor{c000000}{+0.8} & \cellcolor{c587da5} \textcolor{c000000}{+4.6} & \cellcolor{c9cc8e0} \textcolor{c000000}{+2.4} & \cellcolor{c9ec9e1} \textcolor{c000000}{+2.4} & \cellcolor{cf9cab4} \textcolor{c000000}{-1.7} & \cellcolor{c8dbedb} \textcolor{c000000}{+2.7} & \cellcolor{cafd4e7} \textcolor{c000000}{+2.1} & \cellcolor{cd8e9f3} \textcolor{c000000}{+1.2} \\
\lang{vi}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-6.6} & \cellcolor{cf8c5ae} \textcolor{c000000}{-1.9} & \cellcolor{cf5bba4} \textcolor{c000000}{-2.1} & \cellcolor{cfde3d4} \textcolor{c000000}{-1.1} & \cellcolor{c8bbdda} \textcolor{c000000}{+2.7} & \cellcolor{cfde7d9} \textcolor{c000000}{-1.0} & \cellcolor{c699bc8} \textcolor{c000000}{+3.8} & \cellcolor{cb2d6e8} \textcolor{c000000}{+2.0} & \cellcolor{cfde3d4} \textcolor{c000000}{-1.1} & \cellcolor{cfde7da} \textcolor{c000000}{-0.9} & \cellcolor{cb2d6e8} \textcolor{c000000}{+2.0} & \cellcolor{cfde9dd} \textcolor{c000000}{-0.8} & \cellcolor{c9cc8e0} \textcolor{c000000}{+2.4} & \cellcolor{c79b0d3} \textcolor{c000000}{+3.1} & \cellcolor{cecf3f7} \textcolor{c000000}{+0.5} & \cellcolor{ce49385} \textcolor{c000000}{-2.9} & \cellcolor{cb9d9ea} \textcolor{c000000}{+1.8} & \cellcolor{ce1eef5} \textcolor{c000000}{+0.9} & \cellcolor{cf8f9f9} \textcolor{c000000}{+0.1} \\
\midrule
\lang{ar}{MT} & \cellcolor{cd57676} \textcolor{c000000}{-3.5} & \cellcolor{cfcede5} \textcolor{c000000}{-0.6} & \cellcolor{cfcebe1} \textcolor{c000000}{-0.7} & \cellcolor{cfbf2ed} \textcolor{c000000}{-0.4} & \cellcolor{ceda895} \textcolor{c000000}{-2.5} & \cellcolor{ceff5f8} \textcolor{c000000}{+0.4} & \cellcolor{cfde7d9} \textcolor{c000000}{-1.0} & \cellcolor{c506e90} \textcolor{c000000}{+5.0} & \cellcolor{cf9f9f9} \textcolor{c000000}{-0.0} & \cellcolor{cebf3f7} \textcolor{c000000}{+0.5} & \cellcolor{cb4d7e8} \textcolor{c000000}{+2.0} & \cellcolor{cebf3f7} \textcolor{c000000}{+0.5} & \cellcolor{ca7cfe4} \textcolor{c000000}{+2.2} & \cellcolor{c84b9d8} \textcolor{c000000}{+2.8} & \cellcolor{c93c2dd} \textcolor{c000000}{+2.6} & \cellcolor{cfcdac9} \textcolor{c000000}{-1.3} & \cellcolor{cfde4d6} \textcolor{c000000}{-1.0} & \cellcolor{cb5d8e9} \textcolor{c000000}{+2.0} & \cellcolor{cecf3f7} \textcolor{c000000}{+0.5} \\
\lang{bg}{MT} & \cellcolor{cf9c8b2} \textcolor{c000000}{-1.8} & \cellcolor{ca7cfe4} \textcolor{c000000}{+2.2} & \cellcolor{ce6f0f6} \textcolor{c000000}{+0.7} & \cellcolor{cdaeaf3} \textcolor{c000000}{+1.1} & \cellcolor{c5e89b5} \textcolor{c000000}{+4.3} & \cellcolor{c6ca0cb} \textcolor{c000000}{+3.6} & \cellcolor{cddecf4} \textcolor{c000000}{+1.0} & \cellcolor{c5c84af} \textcolor{c000000}{+4.4} & \cellcolor{c74aad0} \textcolor{c000000}{+3.3} & \cellcolor{c8bbdda} \textcolor{c000000}{+2.7} & \cellcolor{c517092} \textcolor{c000000}{+4.9} & \cellcolor{c91c1dc} \textcolor{c000000}{+2.6} & \cellcolor{c537499} \textcolor{c000000}{+4.8} & \cellcolor{c506e90} \textcolor{c000000}{+5.6} & \cellcolor{c54769b} \textcolor{c000000}{+4.8} & \cellcolor{ceaf2f7} \textcolor{c000000}{+0.6} & \cellcolor{c7bb3d5} \textcolor{c000000}{+3.0} & \cellcolor{c608dbc} \textcolor{c000000}{+4.1} & \cellcolor{c7eb5d6} \textcolor{c000000}{+3.0} \\
\lang{el}{MT} & \cellcolor{cdf8a80} \textcolor{c000000}{-3.1} & \cellcolor{ce8f1f6} \textcolor{c000000}{+0.6} & \cellcolor{cedf4f7} \textcolor{c000000}{+0.5} & \cellcolor{ceef4f7} \textcolor{c000000}{+0.4} & \cellcolor{c6c9eca} \textcolor{c000000}{+3.7} & \cellcolor{cd6e8f2} \textcolor{c000000}{+1.2} & \cellcolor{ce7f1f6} \textcolor{c000000}{+0.7} & \cellcolor{c76acd1} \textcolor{c000000}{+3.2} & \cellcolor{cd8e9f3} \textcolor{c000000}{+1.2} & \cellcolor{c7eb5d6} \textcolor{c000000}{+3.0} & \cellcolor{c6798c7} \textcolor{c000000}{+3.9} & \cellcolor{cbcdbeb} \textcolor{c000000}{+1.8} & \cellcolor{c71a6ce} \textcolor{c000000}{+3.4} & \cellcolor{c6da1cc} \textcolor{c000000}{+3.6} & \cellcolor{cafd4e7} \textcolor{c000000}{+2.0} & \cellcolor{cfbf2ed} \textcolor{c000000}{-0.4} & \cellcolor{cb9d9ea} \textcolor{c000000}{+1.8} & \cellcolor{c88bcd9} \textcolor{c000000}{+2.7} & \cellcolor{cbedceb} \textcolor{c000000}{+1.7} \\
\lang{hi}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-7.0} & \cellcolor{cfde4d6} \textcolor{c000000}{-1.0} & \cellcolor{cd97e7a} \textcolor{c000000}{-3.3} & \cellcolor{cf3b69f} \textcolor{c000000}{-2.2} & \cellcolor{ccfe5f0} \textcolor{c000000}{+1.3} & \cellcolor{c8dbedb} \textcolor{c000000}{+2.7} & \cellcolor{cfceee6} \textcolor{c000000}{-0.6} & \cellcolor{cc3dfed} \textcolor{c000000}{+1.6} & \cellcolor{cf8c7b0} \textcolor{c000000}{-1.8} & \cellcolor{cfaf7f5} \textcolor{c000000}{-0.2} & \cellcolor{c506e90} \textcolor{c000000}{+7.0} & \cellcolor{cfceee6} \textcolor{c000000}{-0.6} & \cellcolor{c506e90} \textcolor{c000000}{+5.7} & \cellcolor{ce2eef5} \textcolor{c000000}{+0.9} & \cellcolor{ceef4f7} \textcolor{c000000}{+0.4} & \cellcolor{cd87c79} \textcolor{c000000}{-3.4} & \cellcolor{cd8e9f3} \textcolor{c000000}{+1.1} & \cellcolor{cc3dfed} \textcolor{c000000}{+1.6} & \cellcolor{cf5f7f9} \textcolor{c000000}{+0.2} \\
\lang{ru}{MT} & \cellcolor{cf9cdb8} \textcolor{c000000}{-1.7} & \cellcolor{ce3eff5} \textcolor{c000000}{+0.8} & \cellcolor{cd8e9f3} \textcolor{c000000}{+1.2} & \cellcolor{cc0ddec} \textcolor{c000000}{+1.7} & \cellcolor{c6393c4} \textcolor{c000000}{+4.0} & \cellcolor{ca7cfe4} \textcolor{c000000}{+2.2} & \cellcolor{ccee4f0} \textcolor{c000000}{+1.4} & \cellcolor{c7ab1d4} \textcolor{c000000}{+3.0} & \cellcolor{cb4d7e8} \textcolor{c000000}{+2.0} & \cellcolor{cafd4e7} \textcolor{c000000}{+2.1} & \cellcolor{c537499} \textcolor{c000000}{+4.8} & \cellcolor{c6596c6} \textcolor{c000000}{+3.9} & \cellcolor{c6393c4} \textcolor{c000000}{+4.0} & \cellcolor{c567aa1} \textcolor{c000000}{+4.7} & \cellcolor{c6495c5} \textcolor{c000000}{+4.0} & \cellcolor{cecf3f7} \textcolor{c000000}{+0.5} & \cellcolor{c93c2dd} \textcolor{c000000}{+2.5} & \cellcolor{c6da1cc} \textcolor{c000000}{+3.6} & \cellcolor{c93c2dd} \textcolor{c000000}{+2.5} \\
\lang{ur}{MT} & \cellcolor{c954d62} \textcolor{cf1f1f1}{-8.5} & \cellcolor{cf7bfa7} \textcolor{c000000}{-2.0} & \cellcolor{cab5466} \textcolor{cf1f1f1}{-4.5} & \cellcolor{cd57676} \textcolor{c000000}{-3.5} & \cellcolor{cddecf4} \textcolor{c000000}{+1.0} & \cellcolor{c8fc0dc} \textcolor{c000000}{+2.6} & \cellcolor{cfbd7c5} \textcolor{c000000}{-1.4} & \cellcolor{cfde7d9} \textcolor{c000000}{-1.0} & \cellcolor{cf7c1a8} \textcolor{c000000}{-2.0} & \cellcolor{cfde8dc} \textcolor{c000000}{-0.9} & \cellcolor{c5c86b1} \textcolor{c000000}{+4.4} & \cellcolor{cfcdece} \textcolor{c000000}{-1.2} & \cellcolor{c506e90} \textcolor{c000000}{+6.2} & \cellcolor{ce8f1f6} \textcolor{c000000}{+0.7} & \cellcolor{cf7f8f9} \textcolor{c000000}{+0.1} & \cellcolor{ca75265} \textcolor{cf1f1f1}{-4.6} & \cellcolor{ce5f0f6} \textcolor{c000000}{+0.7} & \cellcolor{ce4eff5} \textcolor{c000000}{+0.8} & \cellcolor{cfcede4} \textcolor{c000000}{-0.7} \\
\lang{th}{MT} & \cellcolor{ccb606c} \textcolor{c000000}{-3.9} & \cellcolor{cfbf4f0} \textcolor{c000000}{-0.3} & \cellcolor{cfad1bd} \textcolor{c000000}{-1.6} & \cellcolor{cfde7da} \textcolor{c000000}{-0.9} & \cellcolor{ccce3ef} \textcolor{c000000}{+1.4} & \cellcolor{ceff5f8} \textcolor{c000000}{+0.4} & \cellcolor{cfaf7f5} \textcolor{c000000}{-0.2} & \cellcolor{cbcdbeb} \textcolor{c000000}{+1.8} & \cellcolor{cfaf6f3} \textcolor{c000000}{-0.2} & \cellcolor{cf9f9f9} \textcolor{c000000}{+0.0} & \cellcolor{ce0edf5} \textcolor{c000000}{+1.0} & \cellcolor{cf8f9f9} \textcolor{c000000}{+0.1} & \cellcolor{cdfedf4} \textcolor{c000000}{+1.0} & \cellcolor{c506e90} \textcolor{c000000}{+5.7} & \cellcolor{c7bb3d5} \textcolor{c000000}{+3.0} & \cellcolor{cf9cdb8} \textcolor{c000000}{-1.7} & \cellcolor{ceaf2f7} \textcolor{c000000}{+0.6} & \cellcolor{cc7e1ee} \textcolor{c000000}{+1.5} & \cellcolor{cecf3f7} \textcolor{c000000}{+0.5} \\
\lang{zh}{MT} & \cellcolor{ceeaa97} \textcolor{c000000}{-2.5} & \cellcolor{cc8e1ee} \textcolor{c000000}{+1.5} & \cellcolor{cfaf5f2} \textcolor{c000000}{-0.2} & \cellcolor{ce1eef5} \textcolor{c000000}{+0.9} & \cellcolor{c55779d} \textcolor{c000000}{+4.8} & \cellcolor{c6596c6} \textcolor{c000000}{+3.9} & \cellcolor{cc8e1ee} \textcolor{c000000}{+1.5} & \cellcolor{c6a9cc9} \textcolor{c000000}{+3.7} & \cellcolor{cd3e7f1} \textcolor{c000000}{+1.3} & \cellcolor{cd1e6f1} \textcolor{c000000}{+1.3} & \cellcolor{c506e90} \textcolor{c000000}{+5.1} & \cellcolor{cb2d6e8} \textcolor{c000000}{+2.0} & \cellcolor{c587ea7} \textcolor{c000000}{+4.5} & \cellcolor{c506e90} \textcolor{c000000}{+5.7} & \cellcolor{c506e90} \textcolor{c000000}{+7.9} & \cellcolor{cfaf8f7} \textcolor{c000000}{-0.1} & \cellcolor{c72a7cf} \textcolor{c000000}{+3.4} & \cellcolor{c6596c6} \textcolor{c000000}{+3.9} & \cellcolor{c88bcd9} \textcolor{c000000}{+2.8} \\
\bottomrule
\end{tabularx}
